Signal Formation in a Detector with one Large Dimension

We present the theory for the signal formation in a multi conductor detector with cylindrical geometry and long length. There exists electromagnetic wave propagation along the large dimension of the detector. The system is equivalent to a multi conductor transmission line. The treatment is in the TEM approximation. Each conductor is fed by its current source which is the same as in the case of small size detectors. A simple example is given for a long length Monitored Drift Tube (MDT). One could apply the result to a long micromegas-type detector or any long microstrip detector, ignoring propagation that is transverse to the strips.

==> Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

The micromegas, an abbreviation for MICRO MEsh GAseous Structure (MM), technology was developed in the middle of the 1990's introducing a micropattern gaseous detector with two asymmetric regions\cite{FirstReference}. Standard MM detectors consist of a planar (drift) electrode, a gas gap of a few millimeters thickness acting as conversion and drift region, and a thin metallic mesh at typically $100-150\,$\textmu m distance from the readout electrode, creating the amplification region, as shown in Figure \ref{fig:mm_principle}. The HV potentials are chosen such that the electric field in the drift region is a few hundred V/cm, and 40$-$50 kV/cm in the amplification region achieving gas gain values of the order of $\mathrm{10^4}$. \\

\begin{figure}[H]
\centering
%\includegraphics[scale=0.12]{plots/mm_structure}
\includesvg{figures/mm_structure}
%\includegraphics[scale=0.3]{plots/mm_principle}
\includesvg{figures/mm_principle}
\caption{Left: MM detector structure of a standard non resistive MM.
chamber Right: Principle of operation for a resistive MM chamber
with readout strips of $400\,\upmu \mathrm{m}$ pitch.}
\label{fig:mm_principle}
\end{figure}

\noindent Charged particles traversing the drift space ionize the gas and the electrons, liberated by the ionization process, drift towards the mesh (in tens of nanoseconds). With an electric field in the amplification region $50-100$ times stronger than the drift field, the mesh is transparent to more than $95\,\%$ of the electrons. The electron avalanche takes place in the thin amplification region in less than a nanosecond, resulting in a fast pulse on the readout strip\cite{ThirdReference}. The drifting of the electrons and the avalanche formation in the amplification region for perpendicular and inclined, with respect to the chamber plane, tracks is illustrated in the right part of Figure \ref{fig:mm_principle}. The ions that are produced in the avalanche process move towards the mesh with velocities about $100$ times smaller than the electrons.

\begin{figure}[H]
\centering
%\includegraphics[scale=0.9]{plots/RMM_structure_side.pdf}
\includesvg{figures/RMM_structure_side}
\caption{Spark Resistant MM. Sketch of the resistive and readout
strip structure.} \label{fig:mm_res}
\end{figure}

\noindent Adding a layer of resistive strips on top of a thin insulator directly above the readout electrode, as shown in Figure \ref{fig:mm_res}, the MM becomes spark-insensitive. The readout electrode is no longer directly exposed to the charge created in the amplification region. The signals on the readout strips are partly induced signals and partly capacitively coupled to it. By adding this protection some fraction of the signal height is lost but the chamber can be operated at higher gas gain because sparking is reduced by about three orders of magnitude\cite{SecondReference}.\\

\noindent The MM technology is quite attractive for High Energy Particle Physics experiments due to its high rate capability, excellent performance and
simplicity of construction. As a result an R$\&$D activity started in 2007, called Muon ATLAS MicroMegas Activity (MAMMA), to explore the potential of the MM
technology for use in LHC experiments. On May 2013 ATLAS decided to equip the New Small Wheel (NSW) with MM detectors\cite{FourthReference}, combining triggering and precision tracking functionality in a single device\cite{JoergReference}.


\begin{figure}[H]
\centering
%\includegraphics[scale=0.03]{plots/mm_tb_h2.jpg}
\includesvg{figures/mm_tb_h2}
%\includegraphics[scale=0.03]{plots/mm_tb_h6.jpg}
\includesvg{figures/mm_tb_h6}
%\includegraphics[scale=0.04]{plots/mm_tb_desy.jpg}
\includesvg{figures/mm_tb_desy}
%\includegraphics[scale=0.049]{plots/sw_mm_picture.png}
\includesvg{figures/sw_mm_picture}
\caption{MAMMA collaboration various test beam activities including
installation in ATLAS (H2, H6, DESY, ATLAS installation).}
\label{fig:mm_tb_h6}
\end{figure}

\noindent Numerous resistive type prototypes of various sizes, and resistivity values have been fabricated over the past years. In addition, a significant amount of time has been invested from the collaboration in testing the operational and performance characteristics of the chambers. Test have been carried out at CERN as well as in other collaborating institutes across Europe with a great number of people being involved. Some photos of the four different setups as well as the chambers installed in the ATLAS cavern are shown in Figure \ref{fig:mm_tb_h6}.\\

\noindent Because of the magnetic field in the ATLAS NSW ($\leq$0.4\,T) region, the study of the MM operated inside a magnetic field has been of particular interest. Such a study has been carried out in the H2 test beam at CERN during June 2012. The effect of the magnetic field on the detector performance is compared to simulation and theoretical expectations based on a simplified model.

%\noindent In addition to analyzing and understanding the test beam data, detailed simulation of the MM chambers has been developed. By comparing the results from data analysis with simulation expectations we were able to finely tune the detectors operational characteristics while, innovative analysis and reconstruction techniques have been developed. Due to the magnetic field in the ATLAS NSW ($\leq$0.4\,T) region, where the MM detector should be able to demonstrate its superb performance characteristics, the study of the MM operated inside a magnetic field has been of particular interest. A dedicated test beam in the H2 CERN north area has been used to study the effect of the field on the detector performance and the results are compared to simulation and to theoretical expectations based on a simplified model.

